An Effective Slope Gap Distribution for Lattice Surfaces

We prove an effective slope gap distribution result first for the square torus and then for general lattice translation surfaces. As a corollary, we obtain a dynamical proof for an effective gap distribution result for the Farey fractions. As an intermediate step, we prove an effective equidistribution result for the intersection points of long horocycles with a particular transversal of the horocycle flow in $\mathrm{SL}_2 (\mathbb R)/\Gamma$ where $\Gamma$ is a lattice.

==> old-effective-estimate.tex <==
\section{Effective Estimates on Transversal}
%\subsection{Effective results on the transversal}
%\label{sec:transversal_counts}



\begin{theorem}[Effective equidistribution on the section]
Let $H_L$ be a the set of points corresponding to a periodic (unstable) horocycle trajectory with unit speed and period $L$. Let $\mathrm{Int_L}$ be the set of intersections of $H_L$ and the Athreya-Cheung section $\Omega$. Let $\rho_{L} = \frac{1}{\lvert \mathrm{Int}_L \rvert}\sum_{x \in \mathrm{Int}_L} \delta_{x}$ and let $m$ be the measure on the section $\Omega$. Let $f \in C_0^{\infty}(\Omega)$. The there exists an $0 < \alpha < 1$ such that \textcolor{red}{Try to prove just for $C_c^{\infty}$-functions first.}

\begin{equation*}
\lvert \rho_L(f) - m(f) \rvert < CL^{-\alpha} \text{.}
\end{equation*}

\noindent \textcolor{red}{How easy is it to upgrade to any interval $I \subset [0,1]$ in the case of Farey fractions?} 
\end{theorem}


%For $f \in C_0^{\infty}(\Omega)$, define $\tilde{f} = f \chi_{[0,\frac{1}{2}]}$, an extension of the function into $G/\Gamma$. The interval is justified on $G/ SL_2(\Z)$ because the return time formula guarantees that a horocycle must spend at least time $t=1$ away from the section before returning. \textcolor{red}{Can we make 1 arbitrary in case this doesn't hold on arbitrary lattice surfaces?}

The main workhorse behind the theorem is ... . To use either, we need our function to be in $C_c^{\infty}(G/\Gamma)$. In order to modify the function so that it is in $C_c^{\infty}(G/\Gamma)$, we need to clip the function so that it is compactly supported, and then smooth it.

Our following goal is to explicitly construct $F_{\varepsilon} \in C_c^{\infty}(G/\Gamma)$ as a smooth approximation of a given $f \in C_0^{\infty}(\Omega)$. 

\begin{comment}

\textbf{Step 1:} Define $f_n \in L^2(\Omega)$ as $f \chi_{R}$ where $R$ is the complement of a cusp region intersected with $\Omega$ with volume $\frac{1}{n^2}$ and whose boundary is a stable horocycle. (Technically, I think $\Omega$ is a cusp region in $\Hh/\Gamma$.)

%\comm{Maybe we can change $K$ to something else, since $K$ can also denote $\mathrm{SO}(2)$ --Tariq}

%\comm{Definitely! I made it $R$. But this will probably all go away in the end anyway.}

To deal with eventual smoothing issues, define

\begin{equation*}
\tilde{f}_{n} = f_n (\chi_{[0,\frac{1}{2}]})
\end{equation*}

\noindent and

\begin{equation*}
\tilde{f} = f (\chi_{[0,\frac{1}{2}]})\text{.}
\end{equation*}



Alternatively: use $\chi_{\frac{1}{n}, \frac{n-1}{n}}$, and define

\begin{equation*}
\tilde{f}_{m,n} = f_m \chi_{[\frac{1}{n},\frac{n-1}{n}]}
\end{equation*}


\noindent Observe that as $n \to \infty$, ${\tilde{f}_{n}}$ approaches $f (\chi_{[0,\frac{1}{2}]})$ at the rate

\begin{equation*}
\int_{G/\Gamma} \left\vert  \tilde{f} - \tilde{f}_n \right\vert \, d\mu \leq \frac{M}{n^2} 
\end{equation*}

\noindent where $M$ is the maximum of the function $f$ in the remainder of the cusp and $\mu$ is the Haar measure on $G/\Gamma$. \textcolor{red}{Do we need to understand the decay rate as they approach infinity? Or is this good enough? How fast do eigenfunctions of $\Delta$ the vanish at infinity decay? See Lang or HT.}

\textbf{Step 2:} Change coordinates to $SL_2(\R)$. 

%\comm{Maybe Iwasawa? --Tariq}

First, recall that in the case of $SL_2(\R)/\SL_2(\Z)$, $\Omega = \lbr (a,b) \in \R^2 : a,b \in (0,1], a + b > 1 \rbr \subset \R^2$. There is an identification with a subset of $SL_2(\R)/SL_2(\Z)$ given by $(a,b) \to \begin{bmatrix} a & b \\ 0 & a^{-1} \end{bmatrix}SL_2(\Z)$. This means that $f$ can be written as 

$$f(n^{-}_{ab} g_{\log{a}}SL_2(\Z)) = f\left(\begin{bmatrix} 1 & ab \\ 0 & 1 \end{bmatrix} \begin{bmatrix} a & 0 \\ 0 & a^{-1} \end{bmatrix}SL_2(\Z)\right)$$ 

\noindent or 

$$f(g_{\log(a)}n^{-}_{\frac{b}{a}}) = f\left(\begin{bmatrix} a & 0 \\ 0 & a^{-1} \end{bmatrix} \begin{bmatrix} 1 & \frac{b}{a} \\ 0 & 1 \end{bmatrix}SL_2(\Z)\right)$$ 

\noindent on the section. 

For the thickened function, $\tilde{f}$, observe that the characteristic function is along an unstable horocycle trajectory. 

For a \textcolor{red}{general cusp region}, we can make the same identification. The transversal $\Omega$ is comprised of cusp regions in $SL_2(\R)/\Gamma$ with \textcolor{red}{(a vertical tangent vector)}. 

\textbf{Step 3:} Smooth the function using a bump function. First, define a metric on $SL_2(\R)$ by pulling back the distance on $T^1(\Hh)$ given by the direct product of the hyperbolic metric and metric on a circle, where we identify the identity element $e$ in $G$ with $i$. Let $d: SL_2(\R) \to \R_{\geq 0}$ denote the distance associate to this metric. Further, let $\lvert \cdot \rvert$ denote the induced norm the Lie algebra. Define $\phi$ to be a bump function centered at the identity in $SL_2(\R)$, 

\begin{equation*}
\phi(g) = \begin{cases} 
      k_1 e^{\left({-\frac{1}{\left( 1 - d(g, e)^2 \right)}}\right)} & d(g, \mathrm{Id}) < k_2 \\
      0 & d(g, \mathrm{Id}) \geq k_2
   \end{cases}
\end{equation*}

\noindent where $k_1$ is such that $\int_{SL_2{\R}} \phi = 1$ and $k_2$ is such that there exists a diffeomorphism between $B_{k_2}(e)$ and a small neighborhood of $0$ in the Lie algebra $\mathfrak{sl}_2{\R}$.

Use this to smooth the function $\tilde{f}_{n}$. Define 

\begin{equation*}
\phi_{\varepsilon}(g) = \frac{1}{\varepsilon^3} \phi\left({\mathrm{exp}\left(\frac{\log(g)}{\varepsilon \lvert \log(g)\rvert}\right)}\right)
\end{equation*}

\noindent where $\mathrm{exp}: \mathfrak{sl}_2{\R} \to  SL_2(\R)$ is the exponential map. Observe that $k_2$ was chosen so that for $g \in \mathrm{supp}(\phi_{\varepsilon})$ is contained in a neighborhood of $0$ such that there is a diffeomorphism between this neighborhood and its image in $SL_2(\R)$.

%\comm{For $\exp$, shouldn't the image be in $\sltr$? -- Tariq} Yep!

Recall the definition of convolution.

\begin{definition}[Convolution]
Let $G$ be a locally compact second countable group with Haar measure $\mu$. Let $f_1: G \to \R$ and $f_2: G \to \R$ be locally integrable functions. The \emph{convolution}, denoted $f_1*f_2$, is

\begin{equation*}
f_1*f_2(g) = \int_G f_1(gh^{-1})f_2(h)\, d\mu(h) = \int_G f_1(h)f_2(h^{-1}g)\, d\mu(h)
\end{equation*}
\end{definition}

Define

\begin{equation*}
F_{\varepsilon} = \phi_{\varepsilon} * \tilde{f}_{n}
\end{equation*}

\noindent where by $*$ we mean convolution. 

Consider the following. \textcolor{red}{Fix. Normalization of the measures!}

\begin{align*}
\rho_L(f) &= \frac{1}{\lvert \mathrm{Int}_L \rvert}\sum_{x \in \mathrm{Int}_L} f(x) \\
&= \left(\frac{1}{\lvert \mathrm{Int}_L \rvert}\sum_{x \in \mathrm{Int}_L} f(x) \right) \left(\frac{2}{L}\int_{H_L} \chi_{[0,\frac{1}{2}]}(s) ds \right)\\
&= \frac{2}{L}\int_{H_L} f(x)(\chi_{[0,\frac{1}{2}]}(s)) d\nu_L(x) ds \\
\end{align*}

\noindent Moreover, let $S$ be the suspension space over $\Delta$, and we have \textcolor{red}{Fix!! Like above.}

\begin{align*}
m(f) &= \int_{\Omega} f dm \\
&= 2 \int_{\Delta} f da db \\
&= \frac{4}{L}\int_{S} f \chi_{[0,\frac{1}{2}]}(s) da db ds. \\
\end{align*}

\noindent Hence, 

\begin{align*}
\left| \rho_L(f) - m(f) \right| &= \left| \frac{2}{L}\int_{H_L} f(x)(\chi_{[0,\frac{1}{2}]}(s)) d\nu_L(x) ds - \int_{\Omega} f dm \right| \\
&\leq \left| \frac{2}{L}\int_{H_L} f(x)(\chi_{[0,\frac{1}{2}]}(s)) d\nu_L(x) ds - \frac{2}{L}\int_{H_L} F_{\varepsilon}(x,s) d\nu_L(x)ds \right| \\
& + \left| \frac{2}{L}\int_{H_L} F_{\varepsilon}(x,s) d\nu_L(x)ds - \frac{4}{L}\int_{S} F_{\varepsilon}(a,b,s) da db ds \right| \\
& + \left| \frac{4}{L}\int_{S} F_{\varepsilon}(a,b,s) da db ds - \frac{4}{L}\int_{S} f \chi_{[0,1/2]} da db ds \right| \\
\end{align*}

The first term on the right hand side can be dealt with by understanding the rate at which the smoothed function approaches the thickened function $\tilde{f}$. The second term can be dealt with by applying a trick by Margulis (or, alternatively, one can use work of Sarnak to produce a the full asymptotic expansion of the decay rate). The last term can also be dealt with by  

The following lemma handles the first term. \textcolor{red}{But not really. It needs some work.}

\begin{lemma} \textcolor{red}{Fix}
\begin{equation*}
\lvert F_{\varepsilon}(g) - \tilde{f}_n(g) \rvert \leq \sup_{d(g,h)< \varepsilon} \lvert \tilde{f}_n(h) - \tilde{f}_n(g) \vert
\end{equation*}
\end{lemma}

\vspace{1cm}

\textcolor{red}{*Might be worth making the bump function less complicated, like Jane suggested.}
\end{comment}

We start with a lemma that allows us to smooth the functions in the parameter space. Below, $\Omega$ denotes the Athreya-Cheung section in $SL_2(\R)/\Gamma$, whereas $\Delta$ denotes the parameter space in $\R^3$. We define $\Delta/\sim$ by identifying edges: \textcolor{red}{top and diagonal}. 

\begin{lemma} $C^{\infty}(\Omega) \cong C^{\infty}(\Delta/ \sim )$, where the smooth structure on $\Delta$ is the smooth structure induced by the ambient $\R^3$. 
\end{lemma}

\begin{proof} Use the map \textcolor{red}{Double check} $\phi: \Delta \to \Omega$ given by $(a,b) \to (\Re(p_{a,b}\cdot i) + i \Im(p_{a,b}^{-1}\cdot i), i)$. Pull back the smooth structure from $\Omega$, and show that this agrees with the usual smooth structure on $\R^3$. \textcolor{red}{We could change $\Delta$ so that $\Phi$ would be $\Phi(a,b) = (p_{a,b}^{-1}\cdot i, i)$, but then we would have to be careful with the corresponding BCZ map. The return map shouldn't really change.}
\end{proof}

Now, let $f \in C_0^{\infty}(\Delta)$. Coordinates in $\Delta$ are given by $(a,b) \in \R^2$. To smooth this function using a bump function from $\R^3$, we need to trim the function away from the edges $\Delta$. Let 

\begin{equation*}
R_{\delta} = \{ (a,b) \in \R^2 : a,b \in (0,1-\delta], a+b > 1 + \delta \}
\end{equation*}

\noindent and define $$f_{\delta} = f \chi_{R_{\delta}} \text{.}$$ Observe that 

\begin{equation}
\int_{\Delta} (f - f_{\delta}) 2dadb \leq 2M_{\delta}\left(3\delta - \left(2 + \frac{1}{\tan(\pi/8)}\right)\delta^2\right)
\end{equation}

\noindent where $M_{\delta} = \max_{x \in \Delta \setminus R_{\delta}}(f(x))$. 

Moreover, for $0 < 2\varepsilon < \delta$, define
%
\begin{equation*}
R_{\delta - \varepsilon} = \{ (a,b) \in \R^2 : a,b \in (0,1 - \delta + \varepsilon], a+b > 1 + \delta - \varepsilon \}
\end{equation*}
%
and
%
\begin{equation*}
R_{\delta + \varepsilon} = \{ (a,b) \in \R^2 : a,b \in (0,1-\delta - \varepsilon], a+b > 1 + \delta + \varepsilon\} \text{.}
\end{equation*}
%

To thicken this function in the parameter space, we need to thicken in the direction of the unstable horocycle. In the parameter space, this manifests as a third coordinate which we will call $s$. Define $$\tilde{f} =  \textcolor{red}{4\zeta(2)} f \chi_{[0, 1/2 ]}$$ and $$\tilde{f}_{\delta} = \textcolor{red}{4\zeta(2)}  f_{\delta} \chi_{[0,1/2]}.$$ Observe that 

\begin{equation}
\int_{S} (\tilde{f} - \tilde{f}_{\delta}) \frac{1}{\zeta(2)}dadbds \leq 2M_{\delta}\left(3\delta - \left(2 + \frac{1}{\tan(\pi/8)}\right)\delta^2\right)
\end{equation}

\noindent where $M_{\delta} = \max_{x \in \Delta \setminus R_{\delta}}(f(x))$. \textcolor{red}{Observe the normalized Haar measure in the suspension space prior to the above statement.}

In order to apply effective equidistribution of long horocycles, we need to smooth the trimmed function. Define $\phi$ to be a bump function centered at $0$ in $\R^3$ such that 

\begin{equation*}
\phi(x) = \begin{cases} 
      k e^{\left({-\frac{1}{\left( 1 - \lvert x \rvert^2 \right)}}\right)} & \lvert x \rvert < 1 \\
      0 & \lvert x \rvert \geq 1
   \end{cases}
\end{equation*}

\noindent where $k$ is such that $\int_{\R^3} \phi dx = 1$. Then, for any $\varepsilon > 0$, define

\begin{equation*}
\phi_{\varepsilon}(x) = \frac{1}{\varepsilon^3} \phi\left(\frac{x}{\varepsilon}\right) \text{.}
\end{equation*}

\noindent We use this bump function to smooth $f_{\delta}$. Fix $\varepsilon$ such that $0 < 2\varepsilon < \delta$. Let $\psi$ be a continuous approximation of $f_{\delta}$ such that $\mathrm{supp}(\psi) = \{ (a,b) \in \R^2 : a,b \in (0,\delta], a+b > 1 + \varepsilon \}$. Then $\int_{\Delta} \left\vert \right\vert 2dadb \leq \varepsilon $



Now, for $0< \varepsilon < \delta$, define $$F_{\varepsilon}= \phi_{\varepsilon}*\psi$$ where by $*$ we mean convolution in $\R^3$. 

Consider the following (\textcolor{red}{reference \ref{thm:intersections-to-length}}, this is derived below the theorem). 

\begin{align*}
\rho_L(f) &= \frac{1}{\lvert \mathrm{Int}_L \rvert}\sum_{x \in \mathrm{Int}_L} f(x) \\
& = 2 \zeta(2) \left( 1 - O \left(\frac{\log(L)}{\sqrt{L}}\right)\right) \frac{1}{L} \sum_{x \in \mathrm{Int}_L} f(x) \\
\end{align*}

\noindent For $\nu_L$ the normalized measure on the horocycle $H_L$ ($\nu_L(H_L) = 1$), we have:

\begin{align*}
\nu_L(\tilde{f}) &= \left(4\zeta(2)\right) \int_{S} f\chi_{[0, \frac{1}{2}]} d\nu_L \\
&= \left(4\zeta(2)\right) \frac{1/2}{L} \sum_{x \in \mathrm{Int}_L} f(x)\\
&= \left(2\zeta(2)\right) \frac{1}{L} \sum_{x \in \mathrm{Int}_L} f(x) \text{.}\\
\end{align*}

\noindent Hence,

\begin{equation}\label{eq:rho-to-nu}
\rho_L(f) = \left( 1 - O \left(\frac{\log(L)}{\sqrt{L}}\right)\right) \nu_L(\tilde{f}).\\
\end{equation}


\noindent Moreover, let $S$ be the suspension space over $\Delta$, and we have

\begin{align*}
m(f) &= \int_{\Omega} f dm \\
&= 2 \int_{\Delta} f da db \\
&= 4 \int_{S} f(a,b) \chi_{[0,\frac{1}{2}]}(t) da db dt. \\
\end{align*}

\noindent 

Now, let $\rho_L, \nu_L$, and $m$ be as above. Let $\mu$ denote the normalized Haar measure on $SL_2{\R}/\SL_2(\Z)$ where $\mu(SL_2(\R)/\SL_2(\Z)) = 1$. Let $f, \tilde{f}$, and $F_{\varepsilon}$ be as above. By the triangle inequality, we have the following. 

%\comm{I think I understand my confusion now. I kept thinking that $\rho_L$ and $\nu_L$ are close as probability measures, but this is not the case, right? Only for $\tilde f$ that are constant in the unstable direction, and so it makes sense to scale this constant in that direction to make these quantities close. --Tariq}

%\comm{Right - and it turns out (since we have equidistribution) that this extra factor shows up when we compare the measure $m$ to the (normalized Haar measure. Hopefully I'll have this written below soon. --Josh}

\begin{align*}\label{eq:term-splitting}
\left| \rho_L(f) - m(f) \right| &\leq \left| \rho_L(f) - \nu_L(\tilde{f}) \right| + \left| \nu_L(\tilde{f}) - \nu_L(F_{\varepsilon}) \right| + \left| \nu_L(F_{\varepsilon}) - \mu(F_{\varepsilon}) \right| \\ 
&\,\,\,\,\, + \left| \mu(F_{\varepsilon}) - \mu(\tilde{f}) \right| + \left| \mu(\tilde{f}) - m(f) \right| 
\end{align*}

For the first term, observe that by Equation \ref{eq:rho-to-nu}

\begin{comment}
\begin{align*}
\left| \rho_L(f) - \nu_L(\tilde{f}_{\delta}) \right| \leq \left| \rho_L(f) - \rho_L(f_{\delta}) \right| + \left| \rho_L(f_{\delta}) - \nu_L(\tilde{f}_{\delta}) \right|.
\end{align*}

\noindent By ergodicity of the BCZ-map and the geometry of $\Delta \setminus R_{\delta}$,  


\begin{align*}
\left| \rho_L(f) - \rho_L(f_{\delta})  \right| &= \frac{1}{\lvert \mathrm{Int}_L \rvert} \sum_{x \in \mathrm{Int}_L} \left( f(x) - f_{\delta}(x) \right)\\
&\leq M_{\delta} \cdot \frac{1}{\lvert \mathrm{Int}_L \rvert} \cdot \lvert \mathrm{Int}_L \cap (\Delta \setminus R_{\delta}) \rvert \\
&\leq M \cdot O(1)(3\delta - (2 + \frac{1}{\tan(\pi/8)})\delta^2)
\end{align*}

\noindent where $M_{\delta} = \max_{x \in \Delta \setminus R_{\delta}}$, and $M$ is a constant independent of $\delta$. \textcolor{red}{May as well pick M to be the max of the function times $2$.} \textcolor{red}{FIX THIS! Not effective. Instead, compare $\rho(L)$ directly to $\nu(L)$.}


\noindent Observe that by Equation \ref{eq:rho-to-nu}:
\end{comment}
%
\begin{align*}
\left| \rho_L(f) - \nu_L(\tilde{f}) \right| \leq O \left(\frac{\log(L)}{\sqrt{L}}\right).
\end{align*}

To handle the last term in Equation \ref{eq:term-splitting}, we use that $\int_S 2dadbds = 2\zeta(2)$, and that $2dadbds$ is the Haar measure~\cite{Athreya-Cheung-poincare-section}. From this, we concluded that the normalized Haar measure in the suspension space (normalized so that $\mu(S) = 1$) is $\frac{1}{\zeta(2)}dadbds$. It follows that 
%
\begin{align*}
\left| \mu(\tilde{f}) - m(f) \right| &= \left| \int_S \tilde{f} \cdot \frac{1}{\zeta(2)}dadbdt - \int_{\Delta} f \cdot 2dadb \right| \\
&= \left| \int_S 4 \zeta(2) f \chi_{[0, 1/2 ]} \cdot \frac{1}{\zeta(2)} dadbdt - \int_{\Delta} f \cdot 2dadb \right| \\
&= \left| \left( 2 \int_0^{\frac{1}{2}} dt \right) \cdot \left( \int_{\Delta} f \cdot 2 dadb \right) - \int_{\Delta} f \cdot 2dadb \right| \\
&= 0 \text{.} \\
\end{align*}

For the third term, we apply Theorem \ref{thm:eff-equid-long-hor-mixing}. For any $\varepsilon > 0$,

\begin{equation*}
\left| \nu_L(F_{\varepsilon}) - \mu(F_{\varepsilon}) \right| \leq \begin{cases} 
      C \mathcal{S}_{K}(F_{\varepsilon}) \log(L) L^{-\frac{1}{2}+ \varepsilon} & \text{if } \Gamma \text{ is tempered}\\
      C(s) \mathcal{S}_{K}(F_{\varepsilon}) L^{-\frac{1}{2}(1-s) + \varepsilon} & \text{if } \Gamma \text{ is non-tempered.}
\end{cases} 
\end{equation*}

For the fourth term, consider the following. We estimate $\tilde{f}$ using the function $\tilde{f}_{\delta}$, and apply the triangle inequality. First the first term below, we split the integral into two pieces, one piece of small measure where the difference between the smoothed cut-off function and the cut-off function is large, and the other piece where the difference between the smoothed cut-off function and cut-off function is controlled by the derivative. Recall our assumption that $f$ is compactly supported, so the sup of $\tilde{f}_{\delta}^{\prime}$ exists over the set we are considering. \textcolor{red}{Fix: Need the unstable parabolic direction.}

\begin{align*}
\left\vert \mu(F_{\varepsilon}) - \mu(\tilde{f}) \right\vert &\leq \left\vert \mu(F_{\varepsilon}) - \mu(\tilde{f}_{\delta}) \right\vert + \left\vert \mu(\tilde{f}_{\delta}) - \mu(\tilde{f}) \right\vert \\
&\leq \int_{S} \left\vert \phi_{\varepsilon} * \tilde{f}_{\delta} - \tilde{f}_{\delta} \right\vert d\mu + \int_S \left\vert \tilde{f}_{\delta} - \tilde{f} \right\vert d\mu\\
&= \int_{R_{\delta - \varepsilon} \setminus R_{\delta + \varepsilon}} \left\vert \phi_{\varepsilon} * \tilde{f}_{\delta}  - \tilde{f}_{\delta} \right\vert d\mu + \int_{ S \setminus (R_{\delta - \varepsilon} \setminus R_{\delta + \varepsilon})} \left\vert \phi_{\varepsilon} * \tilde{f}_{\delta}  - \tilde{f}_{\delta} \right\vert d\mu  \\
&\,\,\,\,\,\,\,\,\,\, + \mu(\mathrm{supp}(\tilde{f} ) \setminus \mathrm{supp}(\tilde{f}_{\delta})) \cdot M_f \\
& \leq \mu(R_{\delta - \varepsilon} \setminus R_{\delta + \varepsilon}) \cdot M_f + \int_{ S \setminus (R_{\delta - \varepsilon} \setminus R_{\delta + \varepsilon})} \sup_{d_{\R^3}(x,y) < \varepsilon} \left\vert \tilde{f}_{\delta}(x) - \tilde{f}_{\delta}(y) \right\vert d\mu \\
&\,\,\,\,\,\,\,\,\,\, + \mu(\mathrm{supp}(\tilde{f} ) \setminus \mathrm{supp}(\tilde{f}_{\delta})) \cdot M_f \\
& \leq \mu(R_{\delta - \varepsilon} \setminus R_{\delta + \varepsilon}) \cdot M_f + \sup_{x \in S \setminus (R_{\delta - \varepsilon} \setminus R_{\delta + \varepsilon})} \tilde{f}_{\delta}^{\prime} + \mu(\mathrm{supp}(\tilde{f} ) \setminus \mathrm{supp}(\tilde{f}_{\delta})) \cdot M_f
\end{align*}

Now consider the second term, $\left| \nu_L(\tilde{f}) - \nu_L(F_{\varepsilon}) \right|$. Observe that there exists a constant $C>0$ such that
%
\begin{equation*}
\left\vert \nu_L(\tilde{f}) - \nu_L(F_{\varepsilon}) \right\vert \leq \frac{CM_{\tilde{f}}}{L} \int_0^L \chi_{\Delta \setminus R_{\delta} \times [0 \times \frac{1}{2}]}(a,b,s) ds
\end{equation*}
%
where $M_{\tilde{f}}$ is the maximum of $\tilde{f}$. Let $\psi(a,b,s)$ be a 
%
\begin{equation*}
\frac{CM_{\tilde{f}}}{L} \int_0^L \chi_{\Delta \setminus R_{\delta} \times [0 \times \frac{1}{2}]}(a,b,s) ds \leq \frac{CM_{\tilde{f}}}{L} \int_0^L \chi_{\Delta \setminus R_{\delta} \times [0 \times \frac{1}{2}]}(a,b,s) ds
\end{equation*}
%

\begin{comment}
\begin{equation*}
\lvert \phi_{\varepsilon}*\tilde{f}_{\delta}(g) - \tilde{f}_{\delta}(g) \rvert \leq \sup_{d(g,h)< \varepsilon} \lvert \tilde{f}_{\delta}(h) - \tilde{f}_{\delta}(g) \vert \text{.}
\end{equation*}

First, for any $0 < 2\varepsilon < \delta$, \textcolor{red}{FIX: need continuous functions/or prove limsup bound on the below using the Lebesgue set of $\tilde{f}_{\delta}$.}


\noindent Hence, 

\begin{align*}
\left| \nu_L(\tilde{f}_{\delta}) - \nu_L(F_{\varepsilon}) \right| &= \left| \int_S \left( \tilde{f}_{\delta} -\phi_{\varepsilon}*\tilde{f}_{\delta} \right) d\nu_L \right|\\
&\leq \\
\end{align*}
\end{comment}
 





\subsection{Effective equidistribution of long horocycles}
\label{sec:closed}
Let $\pi: SL_2(\R) \to L_0^2(SL_2(\R)/\Gamma)$ be the Koopman representation, where $\pi(g)f(x) = f(g^{-1}x)$.    
%
\begin{definition}[$K$-differentiable]
Let $\omega = \begin{bmatrix} 0 & -1 \\ 1 & 0 \end{bmatrix}$ be a generator of the Lie Algebra of $K$. A function $f \in L^2(SL_2(\R)/\Gamma, \mu)$ is called $K$-differentiable if 
%
\begin{equation*}
d(\omega) f := \lim_{h \to 0} \frac{ \pi(\mathrm{exp}(h \omega))f - f}{h}
\end{equation*}
%
\noindent exists, where $h$ is a scalar and the convergence is in $L^2$. 
\end{definition}

\begin{definition}[$\mathcal{S}_K$] 
We say $f$ is a $K$-Sobolev function, denoted $f \in \mathcal{S}_K$, if $f \in L_2(SL_2(\R)/\Gamma)$ and $d(\omega)f \in L^2(SL_2(\R)/\Gamma)$. We endow $\mathcal{S}_K$ with the norm 
%
\begin{equation*}
\mathcal{S}_K(f) = \left(\| f \|_2^2 + \| d(\omega)f \|_2^2 \right)^{\frac{1}{2}}\text{.}
\end{equation*}
%
\end{definition}

We can smooth functions in $SL_2(\R)$. First, define a metric on $SL_2(\R)$ by pulling back the distance on $T^1(\Hh)$ given by the direct product of the hyperbolic metric and metric on a circle, where we identify the identity element $e$ in $G$ with $i$. Let $d: SL_2(\R) \to \R_{\geq 0}$ denote the distance associate to this metric. Further, let $\lvert \cdot \rvert$ denote the induced norm the Lie algebra. Define $\phi: SL_2(\R) \to \R$:

\begin{equation*}
\phi(g) = \begin{cases} 
      k_1 e^{\left({-\frac{1}{\left( k_2^2 - d(g, e)^2 \right)}}\right)} & d(g, \mathrm{Id}) < k_2 \\
      0 & d(g, \mathrm{Id}) \geq k_2
   \end{cases}
\end{equation*}

\noindent where $k_1$ is such that $\int_{G} \phi = 1$ and $k_2$ is such that there exists a diffeomorphism between $B_{k_2}(\mathrm{Id})$ and a small neighborhood of $0$ in the Lie algebra $\mathfrak{sl}_2(\R)$.
%
Now define 
%
\begin{equation*}
\phi_{\varepsilon}(g) = \frac{1}{\varepsilon^3} \phi\left({\mathrm{exp}\left(\frac{\log(g)}{\varepsilon \lvert \log(g)\rvert}\right)}\right)
\end{equation*}

We will convolve $\phi_{\varepsilon}$ with functions to smooth them in $SL_2(\R)$. Recall the definition of convolution.

\begin{definition}[Convolution]
Let $G$ be a locally compact second countable group with Haar measure $\mu$. Let $f_1: G \to \R$ and $f_2: G \to \R$ be locally integrable functions. The \emph{convolution}, denoted $f_1*f_2$, is

\begin{equation*}
f_1*f_2(g) = \int_G f_1(gh^{-1})f_2(h)\, d\mu(h) = \int_G f_1(h)f_2(h^{-1}g)\, d\mu(h)
\end{equation*}
\end{definition}

\begin{theorem}[Effective Equidistribution of Long Horocycles via Mixing]\label{thm:eff-equid-long-hor-mixing} 
Let $\Gamma$ be a non-cocompact lattice subgroup of $SL_2(\R)$ and let $\mu$ be the Haar measure on $SL_2(\R)/\Gamma$ normalized so that $\mu(SL_2(\R)/\Gamma) = 1$.  Let $f \in C_c^{\infty}(SL_2(\R)/\Gamma)$ and let $h\Gamma$ be a periodic point with respect to the unstable horocycle flow. Then \textcolor{red}{for any $\varepsilon >0$}, \textcolor{blue}{Can we remove the periodic condition? i.e, any piece of any horocycle? I've started updating the proof to make this happen.} 

\begin{equation*}
\left| \int_{SL_2(\R)/\Gamma} f(g_t^{-1} N (h\Gamma)) d\nu_{L} - \int_{SL_2(\R)/\Gamma} f( h\Gamma)  d\mu \right| \leq \begin{cases} 
      C \mathcal{S}_{K}(f) \log(L(t)) L(t)^{-\frac{1}{2}+ \varepsilon} & \text{if } \Gamma \text{ is tempered}\\
      C(s) \mathcal{S}_{K}(f) L(t)^{-\frac{1}{2}(1-s) + \varepsilon} & \text{if } \Gamma \text{ is non-tempered}
\end{cases} 
\end{equation*}

\noindent where $\frac{1-s^2}{4}$ is the bottom of the spectrum of the hyperbolic Laplacian on $\Hh/\Gamma$ and $L(t)$ is the length of $g_t{-1} N(h\Gamma)$.  
\end{theorem}

\begin{remark} Sarnak was the first to give a full asymptotic expansion of the decay in~\cite{Sarnak}.  
\end{remark}

We give a short proof of this well-known result in Appendix \ref{appendix:proof-of-effective-equidist} making the Sobolev norm cited clear. The proof provided uses the `Banana Trick', or `Margulis Thickening', pioneered by Margulis in \textcolor{red}{cite thesis? cite Wieser?}. This technique, coupled with the effective mixing of the geodesic flow yields the effective theorem. 

==> old-effective-gaps.tex <==
%\section{Effective Slope Gap Distributions}
%\comm{Maybe just include this in the introduction.}

%In this section, we will use the effective estimates on the transversal that we proved in Section \ref{sec:effective-transversal} to prove effective slope gap distribution results for the square torus and Farey fractions, as well as for general Veech surfaces 

%\subsection{The square torus and Farey fractions}
%\subsection{Veech surfaces}




% Effective proofs of gaps given in the introduction. 

==> old-torus-case.tex <==
\section{Effective Gaps for Torus}

\comm{Should we move this section into the background and effective slope gaps sections?}

\todo{trim and `state' theorems to give structure}

\subsection{The Case of the Torus $\Omega$}

In this case $\Omega_X$ can be written explicitly in coordinates as
\begin{align}
    \Omega := \{p_{a,b} \sltz : a, b \in (0,1], \: a + b > 1\} \subset X_2,\label{eq:poincare-section}
\end{align}
When $\Omega_X$ is viewed as a subset of $T^1(\Hh)$,
\begin{equation}
    \Omega_X = \{(z, \vecv) \in T^1(H) : \im z \geq 1, \vecv = i\},
\end{equation}
(parameterizing $T^1(\Hh) = \Hh \times \{\vecv \in \C : \|\vecv\| = 1\}$).
\todo{include different pictures for $\Omega$.}

\begin{theorem}[\cite{Athreya-Cheung-poincare-section} Theorem 1.1 therein]
    The set $\Omega$ as defined in \eqref{eq:poincare-section} is a Poincar\'e section for the action of $N$ on $X_2$. Furthermore, given $\Lambda := p_{a,b} \sltz$ the first return time $R(a,b) = \min \{s > 0 : h_s \Lambda_{a.b} \in \Omega\}$ is given by 
    \begin{align}
        R (a, b) =  \frac{1}{ab}.
    \end{align}
    The first return map $T : \Omega  \to \Omega$ can be defined implicitly by 
    \begin{align}
        \Lambda_{T(a, b)} = h_{R(a,b)} \Lambda_{a,b}.\label{eq:implicit-first-return}
    \end{align}
    Let $\Omega$ denote the parameter space for $\Omega_X$, then
    \begin{align}
        \Omega = \lbr (a,b) \in \R^2 : a,b \in (0,1], a + b > 1 \rbr \subset \R^2, 
    \end{align}
    then the first return map $T: \Omega \to \Omega$ defined implicitly in \eqref{eq:implicit-first-return} can be shown to be explicitly described by the BCZ map
    \begin{align}
        T(a, b) = \lpar b, -a + \left\lfloor \frac{1 + a}{b}\right\rfloor b\rpar.
    \end{align}
\end{theorem}

%This section of $h_s$ is constructed by taking a particular piece of the unstable foliation $AU$, c.f. \cite{Athreya-Cheung-poincare-section} Section 2.2.1 therein.

\subsubsection{Gap Distribution for Farey Sequence}
Let $\lambda$ be a probability measure on $\R$. Then define
\begin{align}
    \rho_t (A) := \int_\R \ind_A (\Gamma h_s g_t) \:\de \lambda (s) \label{eq:closed-horocycle-measure}
\end{align}

\begin{theorem}[Effective Equidistribution of Long Closed Horocycles]\label{thm:equidistribution-of-long-closed-horocycles}
    Let $\lambda \ll \mathrm{Leb}$ be a probability measure on $\R$. Let $f \in C_c^\infty (X_2)$. Then there exists $\alpha > 0$ such that 
    \begin{align}
        \int_\R f( g_t h_s  \sltz) \:\de \lambda (s) = \int_{X_2} f \de \mu_{\sltr / \sltz} + O(\calS (f) e^{-\alpha t})
    \end{align}
    as $t \to -\infty$.
\end{theorem}
Theorems of this form have a long history. \todo{give a short summary}.

Define
\begin{align}
    \rho_{Q,I} := \frac{1}{N_I(Q)} \sum_{i : \gamma_i \in I} \delta_{T^i(\tfrac{1}{Q}, 1)}.\label{eq:horocycle-hitting-measure}
\end{align}
The following is a direct corollary of the ineffective version of Theorem \ref{thm:equidistribution-of-long-closed-horocycles}.
\begin{theorem}\label{thm:ineffective-section-equidist}
    Let $I = [\alpha,\beta] \subseteq [0,1]$, and $f \in C_b (\Omega)$. Then  
    \begin{align}
        \lim_{Q \to \infty}\int_\Omega f \: \de \rho_{Q,I}   = \int_\Omega f \:\de m.
    \end{align}
\end{theorem}

Let $I = [\alpha,\beta] \subseteq [0,1]$. We define 
\begin{align}
    \calF(Q) &:= \lbr \tfrac{p}{q} \in [0,1] : (p, q) \in \widehat{\Z}^2, \: 0 < q < Q\rbr, \label{eq:Farey-seq} \\
    N_I (Q) &:= |\calF (Q) \cap I|\label{eq:Farey-seq-size}.
\end{align}
It can be shown that $\calF (Q)$ equidistributes on $[0,1]$ as $Q \to \infty$. This naturally motivates the study of the gap distribution.

For each $Q$, we obtain a sequence $(\gamma^{(Q)}_i)$ from the elements of $\calF (Q)$ by simply listing them in increasing order, i.e.
\begin{align}
    \frac{0}{1} = \gamma^{(Q)}_1 < \gamma^{(Q)}_2 = \frac{1}{Q} < \cdots < \gamma^{(Q)}_{N} < \gamma^{(Q)}_{N+1} = \frac{1}{1}.
\end{align}

The goal of the paper is to provide error estimates for Theorem \ref{thm:ineffective-section-equidist}. As an application of this we obtain an effective version of the following theorem.

\begin{theorem}[Corollary 1.8 \cite{Athreya-Cheung-poincare-section}]\label{thm:ineffective-gap-dist}
    As $Q \to \infty$, 
    \begin{align}
        \frac{|\{\gamma_i \in \calF_I (Q) : \tfrac{3}{\pi^2} |I| Q^2 (\gamma_{i + 1} - \gamma_i) \in (c,d)\}|}{N_I (Q)} \to m \lpar R^{-1} \lpar \frac{\pi^2}{3 |I|}(c,d)\rpar\rpar
    \end{align}
\end{theorem}
This theorem follows from Theorem \ref{thm:ineffective-section-equidist}.
We prove an effective version of Theorem \ref{thm:ineffective-gap-dist} via the Margulis' thickening trick, outlined in Section \ref{section:Margulis-thickening}.

\subsection{Applications of Effective Estimates}
The goal of the paper is to provide error estimates for Theorem \ref{thm:ineffective-section-equidist}. As an application of this we obtain an effective version of Theorem \ref{thm:ineffective-gap-dist}

\subsection{Relation to Gap Distribution for Saddle Connections}

Suppose we know,
\begin{equation}\label{eq:omega-equidist}
    \int_\Omega f \: \de \rho_{Q,I}   = \int_\Omega f \:\de m + O_\eps(Q^{-1 + \eps})
\end{equation}
for $f \in C_c^\infty (\Omega)$ %\comm{$E$ is essentially governed by equidist. of long closed horocycles in $X_2$, and probably of the same order} 

In \cite{Athreya-Cheung-poincare-section}, it is shown that
\begin{equation}
    \frac{|\{\gamma_i \in \calF_I (Q) : \tfrac{3}{\pi^2} |I| Q^2 (\gamma_{i + 1} - \gamma_i) \in (c,d)\}|}{N_I (Q)} = \int_\Omega \ind_{R\inv(\frac{\pi^2}{|I| } c, \frac{\pi^2}{|I|} d)}  \: \de \rho_{Q,I}.
\end{equation}
We hope to use \eqref{eq:omega-equidist} in order to provide sharp estimates for the distribution of gaps in the Farey sequence, for large $Q$.

In the torus case, $R\inv (a,b)$ is well understood, given by the region bounded between two parabolas. We want to take $f_\delta$ so that $f_\delta$ whose support is contained in $\ind_{R\inv(a,b)}$, and $\delta = \delta(Q)$. \comm{choosing the support inside the set allows us to avoid issues at the boundary of the parameter space, as josh is doing} 
%\todo{describe this explicitly}. \
\question{How does this work for lattice surfaces. It should be something similar based on previous meetings.}
%To obtain such an estimate, we must smooth $\ind_{(\frac{\pi^2}{|I| c}, \frac{\pi^2}{|I|} d)} \circ R $ so that it is in the appropriate class of functions in order to apply the effective limit theorem. In particular, we should expect that in fact the error depends on the regularity of the approximation taken.
\comm{Ideally we want the following}

%\todo{rework the following in the specific case of the preimage of an interval under the return time map: $R\inv (a,b)$}
\begin{lemma}[`Portmenteau' Theorem]
    Let $\{P_n\}_{n = 1}^\infty, P$ be a probability measures defined on a metric space $(S,d)$. Suppose that for any $f \in C^{\infty}_c(S)$, and any 
    \begin{equation}
        |\int_S f \:\de P_n - \int_S f \:\de P| \leq E_{f,n}.
    \end{equation}
    Then for any compact (or maybe just bounded?), measurable set $A \subseteq S$ whose boundary is of measure zero with respect to $P$, we have
    \begin{equation}
        |P_n (A) - P(A)| \leq ??
    \end{equation}
    \todo{have a more precise error term, accounting for how well we approximate $A$ by a smooth cutoff}
\end{lemma}

\begin{proof}[Proof Idea]
    Let $\varepsilon > 0$, and take $A_\delta$ such that $A \subset A_\delta$ and $P(A_\delta) < P(A) + \varepsilon$. Define a smooth bump function function $f_\delta$ so that
    \begin{enumerate}
        \item $0 \leq f_\delta (x) \leq 1$ for every $x \in S$.
        \item $f_\delta (x) = 1$ for $x \in A$
        \item $f_\delta (x) = 0$ for $x \in S \setminus A_\delta$.
    \end{enumerate}
    Then 
    \begin{equation}
        P_n (A) \leq \int_S f_\delta \: \de P_n \leq \int_S f_\delta \: \de P + E_{f_\delta, n} \leq P(A_\delta) + E_{f_\delta, n} \leq P(A) + \varepsilon + E_{f_{\delta}, n}
    \end{equation}
    In a similar way (i.e. after defining $A'_\delta \subset A$ etc.) we obtain
    \begin{equation}
        P_n(A) \geq \cdots \geq P(A) - \varepsilon - E_{f'_\delta, n}.
    \end{equation}
    Combining these (provided we show that $E_{f'_\delta, n}$ and $E_{f_{\delta}, n}$ are comparable) we have the result.
\end{proof}


\begin{comment}
\subsection{General Approach}
In the end, we want to have an estimate for 
\begin{align}
    \labs\:\int_\Omega f \de \rho_Q - \int f \de \mu_\Omega\:\rabs.
\end{align}
One thing we need to remember to keep track of in the end is how the error really depends on $Q$. The general scheme in my mind is the following, after a bit of adding and subtracting:
\begin{align}
    \labs\:\int_{\Omega} f \de \rho_Q - \int_{T^1\Hh / \Gamma}\tilde f \de \nu_Q\:\rabs + \labs\:\int_{T^1\Hh / \Gamma}\tilde f \de \nu_Q - \int_{T^1\Hh / \Gamma} \tilde f \de \Haar \:\rabs + \labs\:\int_{T^1\Hh / \Gamma} \tilde f \de \Haar - \int_{\Omega} f \de \mu_\Omega\:\rabs
\end{align}
where $\Haar$ is the  Haar measure normalised to be a probability measure on $T^1\Hh / \Gamma$, which is what Josh wrote in the previous section. Effective equidistribution handles the second term, and will give something that explicitly depends on $Q$. The first and last is where our job is, I think. The first should be handled by Jane's calculation. At the moment I am a little confused about the explicit $Q$ dependence there, but maybe this also comes from the effective equidistribution of closed horocycles? For the last one, if we know how to write $T^1\Hh$ in the `stable-geodesic-unstable' cooridnates, then we can make this term small. We can do this in `Iwasawa coordinates' as well, but `thickening' $f$ to $\tilde f$ in the unstable direction seems like a good move.
\end{comment}



==> old-veech.tex <==
\section{Slope Gap Distributions of Veech Surfaces} 

%% Old writing that talked about equidistribution of closed and nonclosed horocycles separately. 
\begin{comment}
\subsection{Effective equidistribution of long non-closed horocycles}


\todo{Rewrite to cite Theorem \ref{thm:eff-equid-long-hor-mixing} instead.}

The theory of slope gap distributions of a translation surface $(X,\omega)$ uses heavily the equidistribution of the horocycle flow on $\sltr/\Gamma$, where $\Gamma = SL(X,\omega)$ is the Veech group of $(X,\omega)$. Depending on whether or not $(X,\omega)$ is periodic under the horocycle flow, an effective gaps result will rely either on an effective equidistribution result for closed horocycles or for non-closed horocycles. 

The closed horocycle result was discussed in Section \ref{sec:closed}. For non-closed horocycles, we will use a result of Str\"{o}mbergsson \cite{Strombergsson}. 

To state this theorem, we let $\Gamma \subset \sltr$ be a \textbf{lattice} in $\sltr$. That is, $\Gamma$ is a discrete subgroup of $\sltr$ such that $\sltr/\Gamma$ has finite Haar measure. With $\sltr$ acting on $\mathbb{H}$ by M\"{o}bius transformations, $\Sigma = \mathbb{H}/\Gamma$ is a hyperbolic surface and there is a natural projection $\pi: \sltr/\Gamma \rightarrow \mathbb{H}/\Gamma$. Because $\Gamma$ was a lattice, $\Sigma = \mathbb{H}/\Gamma$ has finitely many cusps $\eta_1, \ldots, \eta_k$. We can then choose $\mathcal{C}_1,\ldots, \mathcal{C}_k$ to be disjoint neighborhoods of the $k$ cusps. \

The rate of Str\"{o}mbersson's effective distribution result relies on some knowledge of the spectrum of the Laplacian on $\Sigma$. In particular, if there exists a small eigenvalue $\lambda \in (0,\frac14)$, then let $\lambda_1$ be the smallest such eigenvalue and $s_1 \in (\frac12,1)$ be defined so that $\lambda_1 = s_1(1-s_1)$. If no such $\lambda$ exists, then let $s_1 = \frac12$. For each cusp $\eta_i$, let $\lambda_1^{(i)} \in [\lambda_1, \frac14)$, if it exists, be the smallest positive eigenvalue whose eigenfunction has a nonzero constant term at the cusp $\eta_i$. In this case, define $s_1^{(i)} \in (\frac12,1)$ to solve $\lambda_1^{(i)}=s_1^{(i)}(1-s_1^{(i)})$. Otherwise, set $s_1^{(j)}=\frac12$. 

In addition, let $p_0 \in \Sigma = \mathbb{H}/\Gamma$ be any point and let $\|f\|_{W_4}$ denote the $L^2$ Sobolev norm involving up to the $4$th order Lie derivatives. Finally, for $i \in \{1,\ldots, k\}$ and any $p \in \Sigma$, we define $$\alpha_{p,i} = \limsup_{t \rightarrow \infty,\, g_t(p) \in \mathcal{C}_i} \frac{d(g_t(p), p_0)}{t}.$$ Now, we state Str\"{o}mbergsson's theorem. 

\begin{theorem}[\cite{Strombergsson}]
\label{thm:equidistribution-of-nonclosed-horocycles}
Let $p \in \sltr/\Gamma$ be given and define $$\delta_p = \min\left(1-s_1, \min_i(1-\alpha_{p,i})(1-s_1^{(i)})\right).$$
Then, for any $\delta < \delta_p$ and any $f \in C^4(\sltr/\Gamma)$ with $\|f\|_{W_4}< \infty$, we have that $$\frac{1}{T} \int_0^T f(h_t(p))\,dt = \int_{\sltr/\Gamma} f \, d\mu + O(T^{-\delta}).$$
\end{theorem}

As Str\"{o}mbergsson notes in his paper: by the logarithm law for geodesics, $\delta_{p} = 1-s_1$ for almost every $p \in \sltr/\Gamma$. 
\end{comment}

\subsection{Slope gap distributions and the horocycle flow}

In this section, we will outline the proof that almost every Veech translation surface has a limiting gap distribution.

\todo{Add in basic translation surface definitions}

Let $(X,\omega)$ be a translation surface, and let $\Lambda$ be the set of saddle connections of $(X,\omega)$. Following a convention of Athreya, Chaika, and Leli\'{e}vre (\cite{Athreya-Chaika-Lelievre}), we let $$\Lambda_R := \{v=(a,b)\in \Lambda: 0 \leq b \leq a \leq R\}.$$ That is, $\Lambda_R$ denotes the vectors in $\Lambda$ with a positive $\leq R$ horizontal component and slope between $0$ and $1$. We will be concerned with the set of slopes $\mathbb{S}_R$ of this set as $R \rightarrow \infty$. That is, 
$$\mathbb{S}_R := \{\text{slope}(\mathbf{v}) : \mathbf{v} \in \Lambda_R\}.$$
We wish to understand the distribution of $\mathbb{S}_R$ in the interval $[0,1]$ as $R \rightarrow \infty$. In \cite{Veech}, Veech showed that the cardinality $N(R)$ of $\mathbb{S}_R$ grows quadratically, and that $\mathbb{S}_R$ equidistributes in $[0,1]$ as $R\rightarrow \infty$. 

As a finer notion of the randomness of saddle connection directions on $(X,\omega)$, we wish to understand the \textbf{limiting slope gap distribution}. To define the slope gap distribution of $(X,\omega)$, we first order unique slopes of $\Lambda_R$ in increasing order: 

$$0 \leq s_R^{(0)} < s_R^{(1)} < \ldots < s_R^{N(R)-1} \leq 1.$$

We then consider the set of \textbf{renormalized gaps} 

$$\mathbb{G}_R := \{R^2( s_R^{(i)}-s_R^{(i-1)}) : 1 \leq i \leq N(R)\},$$ where the renormalization by $R^2$ is to counter that the expected gap size decays like $R^2$. 

We say that $f:[0,\infty) \rightarrow [0,\infty)$ is the \textbf{slope gap distribution} of $(X,\omega)$ if, for every $a < b$, we have that $$\lim_{R\rightarrow \infty} \frac{|\mathbb{G}_R \cap (a,b)|}{N(R)} = \int_a^b f(x) \, dx.$$ 

\todo{Cite gap distribution literature. Define Veech surface.}

For the rest of this paper, all translation surfaces $(X,\omega)$ are assumed to be Veech surfaces. An algorithm to compute this limiting gap distribution for Veech surfaces was first proved by Uyanik and Work (\cite{Uyanik-Work}), and then was later improved upon by Kumanduri, Sanchez, and Wang (\cite{Kumanduri-Sanchez-Wang}). Upon closer examination, the proofs as written that these algorithms work rely on the Veech surface having a vertical saddle connection. This is because the proofs rely on an equidistribution result for long closed horocycles, and $(X,\omega)$ is periodic under the horocycle flow $h_s$ if and only if it has a vertical saddle connection. Instead, we will modify this proof so that the algorithms work for all Veech surfaces by appealing to the more general equidistribution result given in Theorem \ref{thm:eff-equid-long-hor-mixing}.

Let $h_s : = \begin{bmatrix} 1 & 0 \\ -s & 1 \end{bmatrix}$ denote the (unstable) horocycle flow and let $g_t := \begin{bmatrix} e^{t/2} & 0 \\ 0 & e^{-t/2}\end{bmatrix}$ denote the geodesic flow. Then, the space 
\begin{equation}
    \label{eq:transversal}
\Omega := \{g\Gamma \in \sltr/\Gamma : g\Lambda \text{ contains a short (length $\leq 1$) horizontal saddle connection}\}
\end{equation}
is a transversal for the horocycle flow. $\Omega$ then naturally inherits a measure $m$ from the Haar measure $\mu$ on $\sltr$, such that $dm \, dt = d \mu$, where $t$ is the horocycle direction. We can then define the return time function $R : \Omega \rightarrow \mathbb{R}_+$ by letting $R(x)$ be the return time of $x \in \Omega$ back to $\Omega$ under the horocycle flow $h_s$. We also can define $T : \Omega \rightarrow \Omega$ by letting $T(x) = h_{R(x)}(x)$ to be the first return map of $x$ to $\Omega$ under the horocycle flow. We note that it also makes sense to extend $T$ to a map $\sltr/\Gamma \rightarrow \Omega$ by defining $T$ as $h_s(x)$ for the first $s>0$ for which $h_s(x) \in\Omega$.  

The following theorem is implicit in the paper of Uyanik and Work \cite{Uyanik-Work}. We note that the proof in Uyanik and Work's paper contains a gap and only works as written for the case when $(X,\omega)$ has a vertical saddle connection. We will sketch a proof of this theorem where we fix this gap. 


\begin{theorem}[\cite{Uyanik-Work}]
\label{thm:gaps} 
Let $(X,\omega)$ be a Veech surface and let $f: \mathbb{R}_+ \rightarrow \mathbb{R}_+$ be the distribution of the $h_s$ return time function. That is, $\int_a^b f(x) \, dx = m \{x \in \Omega : a \leq R(x) \leq b\}$. Then, $f$ is the slope gap distribution of almost every surface in the $\sltr$ orbit of $(X,\omega)$. 
\end{theorem}

The key dynamical result needed to prove this theorem is an equidistribution result about a family of long horocycles with varying starting positions. 

\begin{proposition}
\label{prop:renormalized-equidistribution} 
Let $(X,\omega)$ be a Veech surface and $L > 0$. Then, as $R \rightarrow \infty$, the long horocycle segments $h_s(g_{-2\log(R)}(X,\omega)$ for $0 \leq s \leq R^2 \cdot L$ equidistribute in the $\sltr$ orbit of $(X,\omega)$, which is identified with $\sltr/\Gamma$. 
\end{proposition}

\begin{proof}
\comm{This proof assumes that Theorem \ref{thm:eff-equid-long-hor-mixing} works for both periodic and non-periodic horocycle segments.}

Consider a Veech surface $(X,\omega)$, with Veech group $\Gamma = \SL(X,\omega)$. We can then identify the $\sltr$ orbit of $(X,\omega)$ up to equivalence with $\sltr/\Gamma$  by identifying $(X,\omega)$ with the coset $\Gamma \in \sltr/\Gamma$. 

Theorem \ref{thm:eff-equid-long-hor-mixing} is then an effective equidistribution statement for the segments $g_t^{-1}(h_s\Gamma \subset \sltr/\Gamma)$ for $0 \leq s \leq L$ as $t \rightarrow \infty$. Since $g_t h_s = h_{se^{-t}}(g_t)$, it follows by letting $t=2\log(R)$ that the long horocycle segments $h_s(g_{-2\log(R)}(X,\omega))$ for $0 \leq s \leq R^2 \cdot L$ equidistribute in $\sltr/\Gamma$. 

\todo{Compare with notation in Theorem \ref{thm:eff-equid-long-hor-mixing} for portions of horocycles.}
\end{proof}


With this proposition, we can prove the slope gap distribution theorem of Uyanik and Work. 


\begin{proof}[Proof of Theorem \ref{thm:gaps}.] 
% Following Uyanik and Work, we first consider the slope gap distribution of $(X,\omega)$ where $(X,\omega)$ is vertically periodic. In this case, since $(X,\omega)$ is a Veech surface, the $h_s$ orbit of $(X,\omega)$ is periodic and therefore there exists a minimal $s_0$ for which $h_{s_0} \in \SL(X,\omega)$. \todo{Cite result about Veech surfaces and cylinders.}

Let $(X,\omega)$ be a Veech surface. Let $\Lambda_R$ be the set of saddle connections of slope between $0$ and $1$ for which the $x$ coordinate satisfies $0 < x \leq R$. To understand the slope gaps of the set $\Lambda_R$ of saddle connections with $\ell^\infty$ norm less than $R$, we first renormalize $(X,\omega)$ by $g_{-2\log(R)} = \begin{bmatrix} 1/R & 0 \\ 0 & R \end{bmatrix}$ so that the saddle connection vectors of $g_{-2\log(R)} (X,\omega)$ with a short (length $\leq 1$) positive horizontal component and slope between $0$ and $R^2$ are exactly $g_{-2\log(R)}\Lambda_R$. 

Let $T^i(X,\omega) \in \Omega$ for $i \in \mathbb{N}$ be the $i$th intersection of the $h_s$ orbit of $(X,\omega)$ with the transversal $\Omega$. Then, since the horocycle flow preserves slope gaps, the slope gaps of $g_{-2\log(R)}\Lambda_R$ are exactly the first $|\Lambda_R|-1$ return times of the horocycle flow $R(T^i(g_{-2\log(R)}(X,\omega)))$. These are return times of intersections of the $h_s$ orbit of $g_{-2\log(R)}(X,\omega)$ and $\Omega$ for $0 \leq s \leq R^2$. 
% Since $(X,\omega)$ was $h_s$ periodic with period $s_0$, it follows that  $g_{-2\log(R)}(X,\omega)$ is $h_s$ periodic with period $R^2s_0$, the slope gaps of $g_{-2\log(R)}(X,\omega)$ are the return times of the intersection points of the first $1/s_0$ proportion of the length $R^2s_0$ horocycle orbit of $g_{-2\log(R)}(X,\omega)$ with $\Omega$. 

By \ref{prop:renormalized-equidistribution}, the $h_s$ orbit of $g_{-2\log(R)}(X,\omega)$ for $0 \leq s \leq R^2$ equidistributes in $\sltr/\Gamma$ as $R \rightarrow \infty$. Since $\Omega$ is a transversal to the $h_s$ flow and the Haar measure on $\sltr/\Gamma$ can be decomposed as $da \, db \, ds$ \todo{cite something here} where $da \, db$ is Lebesgue measure in local $(a,b)$ coordinates on $\Omega$ and $ds$ is the length measure in the $h_s$ direction, it follows that the intersection points of the $h_s$ orbit of $g_{-2\log(R)}(X,\omega)$ for $0 \leq s \leq R^2$ with $\Omega$ must equidistribute in $\Omega$. 


% Since segments of long horocycles equidistribute \todo{cite the papers that Athreya-Cheung cite in theorem 5.1}, one can show that these intersection points equidistribute in $\Omega$ as $R\rightarrow \infty$. 

This implies that as $R\rightarrow \infty$, the distribution of slope gaps of $g_{-2\log(R)}(X,\omega)$ is $f$, the distribution of the $h_s$ return time function. But the slope gaps of $g_{-2\log(R)}(X,\omega)$ are exactly the renormalized slope gaps of $(X,\omega)$, so $f$ is also the renormalized slope gap distribution of $(X,\omega)$. 



% We now consider the case when $(X,\omega)$ is not vertically periodic. 

% When $(X,\omega)$ is not vertically periodic, we instead appeal to the effective equidistribution of long non-closed horocycle orbits, as proved by Str\"{o}mbergsson and stated in Theorem \ref{thm:equidistribution-of-nonclosed-horocycles}. One subtlety is that we need the long non-closed horocycle orbits $h_s(g_{-2\log(R)}(X,\omega))$ for $0 \leq x \leq R^2$ to equidistribute. Note that as $R$ increases, our long horocycle pieces are based at different points $g_{-2\log(R)}(X,\omega)$, so this equidistribution does not immediately follow from the equidistribution of single non-closed horocycle orbits. 

% Rather, we need the effective equidistribution of Str\"{o}mbergsson's theorem (Theorem \ref{thm:equidistribution-of-nonclosed-horocycles}) to guarantee that our long horocycles beginning at different points still equidistribute. Using the language of Theorem $4.1$, we note that for each $p=g_{-2\log(R)}(X,\omega)$, 

% $$\alpha_{p,i}  = \limsup_{t \rightarrow \infty,\, g_t(p) \in \mathcal{C}_i} \frac{d(g_t(p), p_0)}{t} = \limsup_{\substack{t \rightarrow \infty, \\g_{t-2\log(R)}((X,\omega)) \in \mathcal{C}_i}} \frac{g_{t-2\log(R)}((X,\omega)), p_0)}{t} = \alpha_{(X,\omega),i}$$

% is a constant that only depends on $(X,\omega)$ and is independent of $R$. We can see this by reparametrizing time $T = t - 2 \log(R)$. 

% Thus, $\delta_{p} = \delta_{g_{-2\log(R)}(X,\omega)} = \min\left(1-s_1, \min_i(1-\alpha_{p,i})(1-s_1^{(i)})\right)$ is also independent of $R$. Thus, for a fixed $\delta < \delta_p$, and any $f \in C^4(\sltr/\Gamma)$ with $\|f\|_{W_4}< \infty$, we have that $$\frac{1}{T} \int_0^T f(h_t(g_{-2\log(R)}(X,\omega)))\,dt = \int_{\sltr/\Gamma} f \, d\mu + O(T^{-\delta}).$$ This shows that the long non-closed horocycle orbits $h_s(g_{-2\log(R)}(X,\omega))$ for $0 \leq x \leq R^2$ to equidistribute. The rest of the proof follows as in the periodic case. 
\end{proof}

\begin{remark} We note that the reason that Uyanik and Work's proof implicitly relied on $(X,\omega)$ being vertically periodic is because they cited the equidistribution of long periodic horocycles (\cite{Sarnak}) to show that the $h_s$ intersection points with $\Omega$ equidistributed. For the $h_s$ orbit of $g_{-2\log(R)}(X,\omega)$ for $0 \leq s \leq R^2$ to be part of a periodic horocycle, $g_{-2\log(R)}(X,\omega)$ must be periodic under $h_s$. But in the case when $(X,\omega)$ is a Veech surface this occurs if and only if $g_{-2\log(R)}(X,\omega)$ and therefore $(X,\omega)$ is vertically periodic, which is also equivalent to $(X,\omega)$ having a vertical saddle connection. \todo{Cite something here.}
\end{remark}

\begin{remark} The convention of Athreya-Chaika-Leli\'{e}vre was to let $\Lambda_R$ consist of saddle connections of slope between $0$ and $1$ for which the $x$ coordinate was positive and $\leq R$. The above proof sketch would also work if we defined $\Lambda_R$ to be to be those saddle connections of slope between $0$ and $L$ for any $L > 0$. In particular, in the periodic case, we could let $L$ be the period of $(X,\omega)$ under the horocycle flow. 
\end{remark}



\begin{comment}
\begin{theorem}[\cite{Strombergsson}]
\label{thm:infinitehorocycle} Let $\Gamma$ be a lattice in $\sltr$ and let $p_0 \in \sltr/\Gamma$. Let $0 \leq \alpha < \frac12$. Then for all $p \in \sltr/\Gamma, T \geq 10$, and $f \in C^4(\sltr/\Gamma)$ such that $\|f\|_{W_4} < \infty$ and $\|f\|_{N_\alpha} := \sup_{p \in \sltr/\Gamma}|f(p)| \cdot e^{-\alpha \cdot d(p,p_0)} < \infty$, 
$$\frac{1}{T} \int_0^T f(h_t(p))\,dt = \langle f \rangle + O\left(\|f\|_{W_4}\right) \left(r^{-1/2}\log^3(r+2) + r^{2_1^{(j)}-1} + t^{s_1-1}\right) + O\left(\|f\|_{N_\alpha}\right) \cdot r^{-1/2},$$ where $r = r(p,T) = T\cdot e^{-d(g_{\log T}(p),p_0)}$ and $j=j(p,T)$ is the index of which cusp $g_{\log T}(p)$ is in (if none, then the $r^{s_1^{(j)}-1}$ term is omitted). The implied constants depend on $\Gamma, \alpha,$ and the choice of neighborhoods of the cusps. 
\end{theorem}

We will now apply this theorem to prove Theorem \ref{thm:gaps} in the case where $(X,\omega)$ is not vertically periodic. The key step is to replace the reliance on the equidistribution of long periodic horocycles with a statement about the equidistribution of long nonperiodic horocycles. In this case, the worry is that even though any single nonperiodic horocycle orbit equidistributes, longer and longer horocycle orbits of length $R^2$ starting at different points $g_{-2\log(R)}(X,\omega)$ might not equidistribute. 

For $R \geq 1$, let $p_R := g_{-2\log(R)}(X,\omega)$ be the renormalized $(X,\omega)$. The renormalized slope gaps of $(X,\omega)$ are the return times of of the intersection points of the length $R^2$ horocycle orbit of $p_R=g_{-2\log(R)}(X,\omega)$ with $\Omega$. 

Letting $T = R^2$, Theorem \ref{thm:infinitehorocycle} shows that given the conditions of the theorem and $p_R$ as defined above, the length $T$ horocycle orbits of $p_R$ satisfy the given equidsitribution statement with $r = r(p_R, T) = T \cdot e^{d(g_{\log T} (g_{-\log T} (X,\omega)), p_0)} = T \cdot e^{d((X,\omega),p_0)}$, which is a constant that does not depend on $R$. This shows that there is a uniform rate of equidistribution of the length $T=R^2$ horocycle orbits beginning at $g_{-2\log(R)}(X,\omega)$ to the Haar measure on $\sltr/\Gamma$. The rest of the argument to show Theorem \ref{thm:gaps} follows similarly to the vertically periodic case. 
\end{comment}

\begin{remark} We note that this argument also shows that every element in the $\sltr$ orbit of $(X,\omega)$ also has the same limiting slope gap distribution, since the $h_s$ return time function is an invariant of the $\sltr$ orbit of $(X,\omega)$. 
\end{remark}




\subsection{The slope gap distribution algorithm}
\label{sec:gaps-algorithm}

In Theorem \ref{thm:gaps}, it was established that the slope gap distribution of a Veech translation surface $(X,\omega)$ can be computed if we understand the transversal $\Omega$ to the horocycle flow of elements in the $\sltr$ orbit of $(X,\omega)$ with a short horizontal saddle connection, as well as the horocycle return time function $R : \Omega \rightarrow \mathbb{R}_+$. In this section, we will outline how to parametrize $\Omega$ and some properties of the return time function $R$, and provide some related intuition. For more details, including full proofs of the statements in this section, please see \cite{Uyanik-Work} and \cite{Kumanduri-Sanchez-Wang}. 

We suppose that $(X,\omega)$ is a Veech translation surface with $n < \infty$ cusps. That is, the Veech group $\Gamma = \SL(X,\omega)$ has $n$ conjugacy classes of maximal parabolic subgroups, with each subgroup contributing a cusp to the quotient $\sltr/\Gamma$. We let $\Gamma_1, \ldots, \Gamma_n$ be representatives of these conjugacy classes. 

If $\Lambda(X,\omega)$ is the set of all saddle connection vectors of $(X,\omega)$, then it can be shown that 
$$\Lambda(X,\omega) = \bigcup_{i=1}^m (\Gamma v_i)$$
is the disjoint union of a finite number of $\Gamma$ orbits $\Gamma v_i$ for vectors $v_i \in \mathbb{R}^2$ (see \cite{Athreya-Chaika-Lelievre}). Here, $m \geq n$, where $n$ is the number of cusps of $\sltr/\Gamma$, which is also equal to the number of conjugacy classes of  maximal parabolic subgroups of the Veech group $\Gamma$. For each such parabolic subgroup, there are one or more $v_i$ given by the saddle connections in the eigendirection of the infinite cyclic generator of $\Gamma_i$. 

As a result of this decomposition of the saddle connections $\Lambda(X,\omega)$, the transversal $\Omega$ of surfaces with a short horizontal saddle (as defined in Equation \ref{eq:transversal}) can be naturally broken up into $n$ disjoint pieces, one for each cusp. 

We have that $\Gamma_i \cong \mathbb{Z} \oplus \mathbb{Z}/2$ or $\mathbb{Z} $ depending on whether $-I$ is in or  not in $\Gamma = \SL(X,\omega)$ respectively. We can choose a generator $P_i$ of the infinite cyclic factor that has eigenvalue $\pm 1$, and let $v_i$ be the shortest saddle connection vector of $(X,\omega)$ that is an eigenvector of $P_i$. Then, there exists a $C_i \in \sltr$ such that $$C_iP_iC_i^{-1} = \begin{bmatrix}\pm 1 & \alpha_i \\ 0 & \pm 1 \end{bmatrix},$$ where the sign of $\pm1$ matches with the sign of the eigenvalue of $P_i$ and $C_i  v_i = \begin{bmatrix} 1 \\ 0 \end{bmatrix}.$

It follows that $C_i (X,\omega)$ is in the transversal $\Omega$ because $C_i v_i$ is a short horizontal saddle connection. The idea to parametrize the piece of $\Omega$ corresponding to $\Gamma_i$ is to notice that for a family of matrices $M_{a,b} \in \sltr$ (up to equivalence by $\Gamma$), $M_{a,b}\cdot C_i (X,\omega)$ has a short horizontal saddle connection $M_{a,b}\cdot C_i v_i$. After making some careful choices about which representative matrices $M_{a,b}$ of $\sltr/\Gamma$ to choose, it was shown in \cite{Kumanduri-Sanchez-Wang} that $\Omega$ could be parametrized by pieces $\Omega_i$ for each parabolic subgroup $\Gamma_i$ as follows: 

Consider $C_i(X,\omega)$ with $C_i$ as defined earlier in this section. $C_i(X,\omega)$ has a horizontal saddle connection $C_i v_i = \begin{bmatrix} 1 \\ 0 \end{bmatrix}$ and therefore breaks up into horizontal cylinders (see \cite{Hubert-Schmidt}). Let $y_0 > 0$ be the shortest cylinder height, and let $x_0 > 0$ be the shortest horizontal component of a saddle connection with height $y_0$. Then, $\Omega_i$ is defined in three cases: 
\begin{enumerate}
    \item When $-I \not \in \SL(X,\omega)$, $$\Omega_i := \{(a,b) \in \mathbb{R}^2: 0 \leq a \leq 1, \frac{1-x_0a}{y_0} - \alpha_i a \leq b \leq \frac{1-x_0a}{y_0}.$$
    \item When $-I \in \SL(X,\omega)$ and the eigenvalue of $P_i$ is $1$, then $\Omega_i$ consists of the triangle from case 1 as well as $-1$ times the triangle. 
    \item When $-I \in \SL(X,\omega)$ and the eigenvalue of $P_i$ is $-1$, $\Omega_i$ is the triangle from case 1 with $\alpha_i$ replaced by $2\alpha_i$. 
\end{enumerate}
The shape of these $\Omega_i$ pieces is depicted in Figure \ref{fig:Omega_i}. Then, $\Omega$ consists of a disjoint union of the pieces $$\Omega_i^M := \{M_{a,b} C_i (X,\omega) : (a,b) \in \Omega_i\}.$$ The $\Omega_i$ thus give computationally nice local coordinates for each piece of the transversal $\Omega$. 

\begin{figure}[ht]
\centering
\begin{tikzpicture}
\draw [fill = red!25] (0,1) -- (3,-0.5) -- (3,-4) -- (0,1);
\node at (4.5,0) {$a$};
\node at (0,2.5) {$b$}; 
\node at (-.3, 1) {$\frac{1}{y_0}$};
\draw[thick, <->] (-1, 0) -- (4,0); 
\draw[thick, <->] (0,-4) -- (0,2); 
\draw (3,-.1) -- (3,.1); 
\node at (3,.3) {$1$}; 

\node at (2, .8) {$b = \frac{-x_0}{y_0} a + \frac{1}{y_0}$}; 

\node at (.2, -2.7) {$b = (\frac{-x_0}{y_0}-n) a + \frac{1}{y_0}$}; 
\end{tikzpicture}
\caption{A parametrization of $\Omega_i$, where $n = \alpha_i$ or $2\alpha_i$ depending on whether $-I \in \SL(X,\omega)$ and the eigenvalues of $P_i$.}
\label{fig:Omega_i}
\end{figure}

\begin{remark} The parametrization described here from Kumarduri-Sanchez-Wang (\cite{Kumanduri-Sanchez-Wang}) is modification of the parametrization from Uyanik-Work (\cite{Uyanik-Work}), chosen so that each piece $\Omega_i$ is guaranteed to break up into finitely many polygonal pieces, each with a piecewise real analytic return time function for the horocycle flow $h_s$. This generically did not happen for the parametrization chosen by Uyanik and Work. This finiteness will be useful when we prove properties of the return time function of $h_s$ to $\Omega$. 
\end{remark}

By Theorem \ref{thm:gaps}, the gap distribution of $(X,\omega)$ can then be computed if we understood the return time function $R(x)$ of $h_s$ to $\Omega$ on each $\Omega_i$ in its local coordinates. 

We now describe some key properties of the return time function $R(x)$, many of which are explained in more detail in \cite{Kumanduri-Sanchez-Wang}. The first result we need is the following finiteness result. 

\begin{proposition}[\cite{Kumanduri-Sanchez-Wang}]
\label{prop:finiteness}
Each piece $\Omega_i$ of the transversal $\Omega$ breaks up into finitely many convex polygonal pieces. On each polygonal piece, there is a single vector $w_i = \begin{bmatrix} x \\ y \end{bmatrix}$ with $y > 0$ of $C_i(X,\omega)$ for which $M_{a,b}w_i$ has the smallest positive slope among all holonomy vectors with a horizontal length component of $\leq 1$. Then, the return time function at the point $(a,b) \in\Omega$ is given by $$R(a,b) = \frac{y}{a(ax+by)},$$ the slope of $M_{a,b}w_i$. On $\Omega_i$, $R(a,b)$ takes values in $(0,\infty)$. 
\end{proposition}

This idea of the return time function  is that $R(a,b)$ is the amount of time needed for the horocycle flow to pull the vector $M_{a,b}w_i$ down to become a short horizontal saddle connection so that $h_sM_{a,b}C_i (X,\omega)$ is in $\Omega$. 


\comm{R(a,b) doesn't seem to be continuous. Will this be a problem?}

We now wish to understand how small and how large $R(a,b)$ can be on each piece $\Omega_i$ of the transversal. 

\begin{proposition} On each piece $\Omega_i$ of the transversal $\Omega$, the return time function $R(a,b)$ is bounded below by some constant $c_i > 0$. 
\end{proposition}
\begin{proof}
By Proposition \ref{prop:finiteness}, $\Omega_i$ breaks into finitely many polygonal pieces on which $R(a,b) = \frac{y}{a(ax+by)}$ for some $x \in \mathbb{R}$ and $y > 0$. On each of these pieces, the return time function is continuous and takes values in $(0,\infty)$. But $\overline{\Omega_i}$ is compact and so the denominator $a(ax+by)$ is bounded above by some $0 < M < \infty$ on the polygonal piece. Since $y > 0$ is fixed, $R(a,b)$ is then bounded below by $\frac{y}{M}> 0$. Taking $c_i$ to be the minimum of these bounds over all of the polygonal pieces, $R(a,b) > c_i > 0$ on all of $\Omega_i$
\end{proof}

\comm{Is it also necessary to know where $R(a,b)$ can go to infinity?}


\subsection{Effective results}

Given $(X,\omega)$ a translation surface, we let $p_R := g_{-2\log(R)}(X,\omega)$ be the renormalized surface. Let $\gamma_R$ denote the horocycle orbit $h_s(p_R)$ for $0 \leq s \leq R^2$. Then, define the measure $\rho_R$ on $\Omega$ as $$\rho_R := \frac{1}{|\gamma_R \cap \Omega|} \sum_{x \in \gamma_R \cap \Omega} \delta_x,$$ the counting measure on $\gamma_R \cap \Omega$. We also let $\nu_R$ be a measure on $\sltr/\Gamma$ that is the measure supported on $\gamma_R$ and normalized so that $\nu_R(\sltr/\Gamma)=1$. We also let $m$ be Lebesgue measure on $\Omega$, which is $da \, db$ in local coordinates on each piece of $\Omega$, normalized so that $m(\Omega) = 1$. Finally, we let $\mu$ be Haar measure on $\sltr/\Gamma$. 


\subsection{Horocycle length and intersection point bounds}


One step in obtaining an effective slope gap distribution result for saddle connections on square torus, and by extension for Farey fractions, is to compare the length of particular horocycle orbits and the number of times those orbits intersect the transversal $\Omega$. In this section, we extend this discussion to the case of Veech surfaces. 


We recall that in the context of computing gap distributions of an arbitrary Veech surface, we let $(X,\omega)$ be a Veech surface with Veech group $\Gamma \subset \sltr$ and $\Omega \subset \sltr/\Gamma$ be the transversal consisting of surfaces with a short (length $\leq 1$) horizontal saddle connection. We follow the convention of Athreya-Chaika-Leli\'{e}vre and let $\Lambda_R(X,\omega)$ consist of saddle connections of slope between $0$ and $1$ for which the $x$ coordinate is positive and $\leq R$. For $R\geq 1$, we let $p_R := g_{-2\log(R)}(X,\omega)$ be the renormalized $(X,\omega)$. 

We let $\gamma_R$ denote $h_s(p_R)$ for $0 \leq s \leq R^2$, the length $R^2$ horocycle starting at the point $p_R$. We wish to compare $\ell(\gamma_R)$, which is $R^2$, with $|\gamma_R \cap \Omega|$, the number of times that $\gamma_R$ intersects the transversal $\Omega$. We note that $\ell(\gamma_R)$ is the analog of $\ell(\gamma_Q)$ in the context of the square torus and Farey fraction discussion in Section \ref{sec:transversal_counts}.  To estimate the latter quantity $|\gamma_R \cap \Omega|$, we will apply the following result of Burrin, Nevo, R\"{u}hr, and Weiss:

\todo{Highlight that this rate is important to our rate, so improving this rate would be consequential. }
\begin{theorem}[\cite{Burrin}, Theorem 2.7]
\label{thm:saddle-counts} 
Let $\Gamma$ be a noncompact lattice in $\sltr$, and let $Y =\Gamma v$ be the $\Gamma$ orbit of a nonzero vector $v$. Let $S$ be a star-shaped domain with a non-negative piecewise Lipschitz boundary curve $\rho(\theta)$, and let $R \cdot S$ be the dilation of $S$ by $R > 0$. Then, for all $\epsilon > 0$, $$|Y \cap R\cdot S| = C_{Y,S} R^2 + O(R^{q_\Gamma + \epsilon}),$$ where the implicity constants on the $O$ term depend on $\Gamma, Y,S,$ and $\epsilon$, and $q_\Gamma$ depends on the spectral gap of the automorphicm representation of $G$ on $L_0^2(G/\Gamma)$. 
\end{theorem}

Using the language of this theorem, we then have the following result. 

\begin{proposition} Let $(X,\omega)$ be a Veech surface and let $p_R := g_{-2\log(R)} (X,\omega)$. Let $\gamma_R$ denote the horocycle orbit $h_s(p_R)$ for $0 \leq S \leq R^2$. Then, using the language of Theorem \ref{thm:saddle-counts},  $$|\gamma_R \cap \Omega| =  c R^2 + O(R^{q_\Gamma + \epsilon})$$ where   $c = \frac{1}{\text{covolume}(\Gamma)}$ and the implicit constant in the $O$ term depends on $(X,\omega)$ and $\epsilon$.
\end{proposition}

\begin{proof}

This horocycle $\gamma_R$ intersects the transversal exactly when $h_s(p_R)$ has a short horizontal saddle connection. Since $h_s$ acts on $(X,\omega)$ via a vertical sheer, the number of intersections is then equal to the number of slopes of saddle connections vectors of $p_R$ that reside in the triangle with vertices at $(0,0), (1,0),$ and $(1,R^2)$. Since $p_R = g_{-2\log(R)}(X,\omega)$, by multiplying by $g_{2\log(R)}$, this is equal to the number of slopes of saddle connections vectors of $(X,\omega)$ in the triangle with vertices at $(0,0), (R,0),$ and $(R,R)$. Figure \ref{fig:renormalization} depicts the effect of renormalization on the relevant saddle connections. 


\begin{figure}[ht]
\centering
\begin{tikzpicture} 

\draw (-1,0) -- (3,0);
\draw (0,-1) -- (0,5);
\draw[fill=blue!25] (0,0) -- (2,0) -- (2,2)  -- (0,0);
\draw (4,0) -- (8,0);
\draw (5,-1) -- (5,5); 
\draw[fill = blue!25] (5,0) -- (6,0) -- (6,4) -- (5,0);
\draw[thick, ->] (3,2) -- (4,2);
\draw node at (3.5, 2.5) {$g_{-2 \log(R)}$};
\draw node at (2,-0.3) {$R$};
\draw node at (-0.3,2) {$R$};
\draw node at (6,-0.3) {$1$};
\draw node at (4.7, 4) {$R^2$};

\draw[dashed] (0,0) -- (1.8,1.6); 
\draw[dashed] (0,0) -- (1.6,0.6); 
\draw[dashed] (0,0) -- (1.4,0.2); 
\draw[dashed] (0,0) -- (0.8,0.6); 

\draw[fill] (1.8,1.6) circle [radius = 0.025]; 
\draw[fill] (1.6,0.6) circle [radius = 0.025]; 
\draw[fill] (1.4,0.2) circle [radius = 0.025]; 
\draw[fill] (0.8,0.6) circle [radius = 0.025]; 

\draw[dashed] (5,0) -- (5.9,3.2); 
\draw[dashed] (5,0) -- (5.8,1.2); 
\draw[dashed] (5,0) -- (5.7,0.4); 
\draw[dashed] (5,0) -- (5.4,1.2); 

\draw[fill] (5.9,3.2) circle [radius = 0.025]; 
\draw[fill] (5.8,1.2) circle [radius = 0.025]; 
\draw[fill] (5.7,0.4) circle [radius = 0.025]; 
\draw[fill] (5.4,1.2) circle [radius = 0.025]; 

\node at (1, -1.5) {$(X,\omega)$};
\node at (6, -1.5) {$p_R = g_{-2\log(R)}(X,\omega)$};
\end{tikzpicture}
\caption{The saddle connections $\Lambda_R$ on the surface $(X,\omega)$ on the left and the transformed saddle connections on $p_R$ on the right.}
\label{fig:renormalization}
\end{figure}

Thus, the number of intersections of the horocycle segment $\gamma_R$ with $\Omega$ for $0 \leq s \leq R^2$ is exactly the number of unique slopes of vectors in 
$$\Lambda_R(X,\omega) = \{\text{saddle connections of } (X,\omega) \text{ with slope in } [0,1] \text{ and $x$ coordinate in } (0,1]\}.$$ 

In Section \ref{sec:gaps-algorithm}, we discussed that the set of all saddle connection vectors of $(X,\omega)$ can be decomposed as 
\begin{equation}
\label{eq:gamma-orbits}
    \Lambda(X,\omega) = \bigcup_{i=1}^m (\Gamma v_i),
\end{equation}
the disjoint union of a finite number of $\Gamma$ orbits $\Gamma v_i$. 

Let $S$ be the triangle in $\mathbb{R}^2$ with vertices at $(0,0), (1,0),$ and $(1,1)$. We wish to count $|\gamma_R \cap \Omega|$, which is equal to the number of unique slopes of $\Lambda_R (X,\omega) = \Lambda(X,\omega) \cap R\cdot S$. In Equation \ref{eq:gamma-orbits}, two saddle connections are in the same direction if and only if they are $\gamma v_i$ and $\gamma v_j$ for $v_i \neq v_j$ in the same direction (corresponding to the same cusp). Upon relabeling, we can take $v_1, \ldots, v_n$ to be a subset of the $v_i$'s that contains one vector for each cusp. Thus, we have that 
\begin{equation} 
\label{eq:gammaR-orbits}
|\gamma_R \cap \Omega| = |\text{unique slopes in } \Lambda_R(X,\omega)| = \left| \bigcup_{i=1}^n (\Gamma v_i) \cap (R\cdot S)\right|.
\end{equation}

We notice that $\bigcup_{i=1}^n (\Gamma v_i) \cap (R\cdot S) \subset \Lambda_R(X,\omega)$ contains exactly one saddle connection with each possible saddle connection slope direction in $\Lambda_R(X,\omega)$. 

 Then, Theorem \ref{thm:saddle-counts} gives us that  for each $v_i$, $$|\Gamma v_i \cap R\cdot S| = C_{\Gamma, v_i, S} R^2 + O(R^{q_\Gamma+\epsilon}).$$ By applying the decomposition from Equation \ref{eq:gammaR-orbits} and summing over the contributions of each $v_i$, we have that  
 \begin{equation} 
 \label{eq:int-counts}
 |\gamma_R \cap \Omega| = |\Lambda_R| = \sum_{i=1}^n |\Gamma v_i \cap R\cdot S| = c R^2 + O(R^{q_\Gamma + \epsilon})
 \end{equation} 
 where $c$ depends on $\Gamma, S, v_1, \ldots, v_n$ and the constant in the $O$ term depends on $\Gamma, v_1, \ldots, v_n,$ and $\epsilon$. 

To determine $c$, we recall that the measures $m, \rho_R, \nu_R, $ and $\mu$ as defined in Section \todo{include reference} are related. We let $f$ be any function on $\Omega$. For a given $(X,\omega)$, by Section \ref{sec:gaps-algorithm}, we can find an $M > 0$ such that the return time of $h_s$ on the transversal $\Omega$ is everywhere $> M$. We then define $\tilde{f}$ by $\tilde{f}(a,b,t) = \frac{1}{M} f(a,b) \chi_{[0,M]}(t)$ where $(a,b)$ are local coordinates on each piece of $\Omega$ as defined in Section \ref{sec:gaps-algorithm} and $t$ is the coordinate in the horocycle direction. 

Following similar logic as when we derived Equation \ref{eq:Q-integrals}, 
\begin{equation}
    \label{eq:R-integrals}
\int_\Omega f \, d\rho_R = \frac{1}{|\{\gamma_R \cap \Omega\}|} \sum_{x \in \gamma_R \cap \Omega} f(x), \text{ and} \int_{\sltr/\Gamma} \tilde{f} \, d\nu_R = \frac{1}{|\ell(\gamma_R)|} \sum_{x \in \gamma_R \cap \Omega} f(x).
\end{equation}

We see then that 
\begin{equation}
    \label{eq:horocycle-integrals}
\int_\Omega f \, d\rho_R = \frac{|\ell(\gamma_R)|}{|\{\gamma_R \cap \Omega\}|} \int_{\sltr/\Gamma} \tilde f \, d\nu_R \xrightarrow{R \rightarrow \infty} \frac{1}{c} \int_{\sltr/\Gamma} \tilde f \, d\nu_R
\end{equation} 
by Equation \ref{eq:int-counts} and since $|\ell(\gamma_R)| = R^2$. 

As shown in the proof of Theorem \ref{thm:gaps}, by equidistribution results for the horocycle flow, $\rho_R$ converges to Lebesgue measure $m$ on $\Omega$, normalized so $m(\Omega) = 1$, and $\nu_R$ converges to Haar measure $\nu$, where $\nu(\sltr/\Gamma) = \text{covolume}(\Gamma)$ is not necessarily $1$. Thus, by taking $f$ to be the constant function that is $1$ everywhere on $\Omega$, and $R \rightarrow \infty$, we have that $$1= \int_\Omega f \,dm = \frac{1}{c} \int_{\sltr/\Gamma} \tilde{f} \, d \mu = \frac{1}{c} \text{covolume}(\Gamma). $$ It then follows that $c = \text{covolume}(\Gamma)$. 
\end{proof}

We can then use this asymptotic to compare $|\gamma_R \cap \Omega|$ with $\ell(\gamma_R) = R^2$.  


 

% \comm{Think about whether these orbits are disjoint. I think that this is mentioned in the golden L paper. Also, include some background on this decomposition of saddle connections into $\Gamma$ orbits result.}

% \comm{Yeah, you can find a basis of vectors whose Veech group orbit is the full set of holonomy vectors in the plane (I think this is in the 89 Veech Eiseinstein series paper). Disjointness of orbits should follow from the fact that they are each orbits of the same group acting on $\mathbb{\R}^2$. In the golden L paper, they seem to recognize that two vectors are all that is needed (I don't know how to deduce this - maybe Veech explains?), and since the two vectors are collinear, they only work with one. I suppose they are defining a ``primitive" set of saddle connections in this way. --Josh}



\comm{To compare the rate at which the two measures $\rho_L$ and $\nu_L$ approach each other against the rate we get from effective equidistribution of long horocycles, we should probably know $q_{\Gamma}$ in both the tempered and non-tempered case. Perhaps its not important if we only want our result to say something like ``there exists a number $\alpha$ less than 1 such that ... $\leq CL^{-\alpha}$". We could give an explicit decay rate for the case of the torus, and then in the general case, indicate that the terms are computable, etc. -- Josh}


\todo{Address what $q_\Gamma$ is.}






==> questions.tex <==
\section{The Plan + Things to sort out}

\begin{enumerate}
    \item Notation and Background
    \item Equidistribution on the big space (maybe make the proof an appendix? Thoughts? -Tariq)
    \item Torus case: Equidistribution on the section + application to gaps.
    \item Generalisation to lattice surfaces.
\end{enumerate}

\begin{comment}
\begin{question}
    Which version of Sarnak's theorem are we using? \\ \: \\
    \comm{For now I have put the version from Andreas' notes, in Theorem \ref{thm:equidistribution-of-long-closed-horocycles}. Beware of how we parameterize the geodesic flow. The exponential decay might be misleading. --Tariq}
    
    \comm{Would it be okay if we quotient on the other side in Theorem \ref{thm:equidistribution-of-long-closed-horocycles}? I wrote this out in my notes, quotiented on the other side. I'd be happy to swap it. For whatever reason, I also used 2s-out notation instead of 2's in. Either way is good for me. --Josh}

    \comm{I swapped it. I also usually quotient on the left, I'm not sure why I did it the other way around now. Note that by switching it, we will need to take $t \to -\infty$ for the horocycle to expand.
    By the way, what's 2's out? Is that $\SL (2, \R)$ vs $\sltr$?--Tariq}
    
    \comm{Ah, $\begin{bmatrix} e^t & 0 \\ 0 & e^{-t}\end{bmatrix}$ (2's out) versus $\begin{bmatrix} e^\frac{t}{2} & 0 \\ 0 & e^-\frac{t}{2}\end{bmatrix}$(2's in) --Josh}
    
    \comm{Ohhhhhh --Tariq}
\end{question}
\end{comment}

\begin{question}[Answered, more or less]
    Is the error term for the equidistribution on the section really exponential, or should it be polynomial? Note that in the effective equidistribution we have the height of the horocycle is controlled $g_t$, so the error term seems better than it is.
\end{question}

\begin{comment}
\begin{question}
    Is the advantage of $K$-invariance to pretend we can just apply harmonic analysis on $\Hh$ as opposed to $T^1 (\Hh)$? Though, making things $K$ invariant might make detecting the section difficult?
\end{question}    
\end{comment}


\begin{question}
    Is it reasonable/standard practice to define the slope gap distribution only for saddle connections of slopes between 0 and 1? 
\end{question}

\comm{I think the answer to this is yes, when the surface is not vertically periodic. When vertically periodic, it also seems reasonable to consider slopes between $0$ and the $h_s$ period. -- Jane}



\begin{question}
    In many papers they state that the tail of the limiting distribution decays quadratically, however the statement is always as an asymptotic. Is it possible to make this more precise? I suspect in the case of the Golden L paper it is, since the description of the limit distribution is explicit (is it also explicit for the geneneric case?). If we can make it more precise, can we then use the effective statement to find the tail decay in terms of $Q$? This might be an interesting application of the effective result we obtain. 

    (Update 1) Maybe this is hard to do in general, but probably we can do it in the torus case where the return time function is explicit.
\end{question}
